Physics Simulation Via Quantum Graph Neural Network

We develop and implement two realizations of quantum graph neural networks (QGNN), applied to the task of particle interaction simulation. The first QGNN is a speculative quantum-classical hybrid learning model that relies on the ability to directly utilize superposition states as classical information to propagate information between particles. The second is an implementable quantum-classical hybrid learning model that propagates particle information directly through the parameters of $RX$ rotation gates. A classical graph neural network (CGNN) is also trained in the same task. Both the Speculative QGNN and CGNN act as controls against the Implementable QGNN. Comparison between classical and quantum models is based on the loss value and accuracy of each model. Overall, each model had a high learning efficiency, in which the loss value rapidly approached zero during training; however, each model was moderately inaccurate. Comparing performances, our results show that the Implementable QGNN has a potential advantage over the CGNN. Additionally, we show that a slight alteration in hyperparameters in the CGNN notably improves accuracy, suggesting that further fine tuning could mitigate the issue of moderate inaccuracy in each model.

==> extra_biblio.tex <==
%@ARTICLE{Giovannetti,
%   author       = "Vittorio Giovannetti and Seth Lloyd and Lorenzo %Maccone",
%   title        = "Quantum random access memory",
%   year         = "2008",
%   journal      = "Physical Review Letters"
%}

%@MISC{Seigelwax,
%   author      = "Brian Seigelwax",
%   title       = "Quantum Memory: QRAM. What is it and why do we need %it? Making Quantum Algorithms Thrive.", 
%   howpublished = "https://quantumzeitgeist.com/quantum-memory-qram-%what-is-it-and-why-do-we-need-it/", 
%   year         = "2022"
%}

%@ARTICLE{Stas,
%   author       = "P.-J. Stas and et al",
%   title        = "Robust multi-qubit quantum network node with %integrated error detection",
%   year         = "2022",
%   journal      = "npj Quantum Inf",
%   volume       = "8",
%   issue        = "122"
%}

%@ARTICLE{Ye,
%   author       = "Y-H Ye and et al",
%   title        = "Long-lived storage of orbital angular momentum %quantum states",
%   year         = "2022",
%   journal      = "Phys. Rev. Lett.",
%   volume       = "129",
%   issue        = "19"
%}

@MISC{Qiskit, 
   title       = "Open-Source Quantum Development", 
   howpublished = "https://qiskit.org/", 
   year         = "2022"
}
